Ranked List Truncation for Large Language Model-based Re-Ranking

We study ranked list truncation (RLT) from a novel "retrieve-then-re-rank" perspective, where we optimize re-ranking by truncating the retrieved list (i.e., trim re-ranking candidates). RLT is crucial for re-ranking as it can improve re-ranking efficiency by sending variable-length candidate lists to a re-ranker on a per-query basis. It also has the potential to improve re-ranking effectiveness. Despite its importance, there is limited research into applying RLT methods to this new perspective. To address this research gap, we reproduce existing RLT methods in the context of re-ranking, especially newly emerged large language model (LLM)-based re-ranking. In particular, we examine to what extent established findings on RLT for retrieval are generalizable to the "retrieve-then-re-rank" setup from three perspectives: (i) assessing RLT methods in the context of LLM-based re-ranking with lexical first-stage retrieval, (ii) investigating the impact of different types of first-stage retrievers on RLT methods, and (iii) investigating the impact of different types of re-rankers on RLT methods. We perform experiments on the TREC 2019 and 2020 deep learning tracks, investigating 8 RLT methods for pipelines involving 3 retrievers and 2 re-rankers. We reach new insights into RLT methods in the context of re-ranking.

==> Sections/09_Backups.tex <==



\begin{table}[!t]
\centering
\caption{
A comparison of \ac{RLT} methods, optimized for re-ranking effectiveness/efficiency tradeoffs, in predicting re-ranking cut-off points for the BM25--RankLLaMA pipeline on TREC-DL 19 and 20.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l lll lll} 
\toprule
 \multirow{2}{*}{Method} & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \multicolumn{1}{c}{Avg. k} & \multicolumn{1}{c}{nDCG@10}     & \multicolumn{1}{c}{Lat.}  & \multicolumn{1}{c}{Avg. k}   & \multicolumn{1}{c}{nDCG@10}    & \multicolumn{1}{c}{Lat.}     \\
\midrule
w/o re-ranking & -  & 0.506    & -   & -   & 0.480  &  -  \\
  \midrule
  Fixed-$k$ (10)  & 10   & 0.557    &  & 10  &  0.532  &      \\
  Fixed-$k$ (20) & 20   & 0.651    &  &  20 & 0.612   &  \\
  Fixed-$k$ (100) & 100  & 0.730    &  & 100  & 0.697  &    \\
  Fixed-$k$ (200) & 200  & 0.739   &  & 200  & 0.719  &   \\
 %$k=300$ & 300  & 0.739   &  & 300 & 0.731  &    \\
 %$k=400$ & 400  & 0.741    &  & 400  & 0.733  &  \
 %$k=500$ & 500   & 0.745   &  & 500 & 0.739  &   \\
% $k=600$ & 600  &  0.743    &  & 600 & 0.750  &   \\
 Fixed-$k$ (1000)  & 1000 & 0.747    &  & 1000  &  0.762 &  \\
Greedy-$k$  &      &       &  &    &       &      \\
Surprise &      &       &  &    &       &   \\
\midrule
BiCut ($\alpha$=0.40)  &      &      &      &   &         &   \\
BiCut ($\alpha$=0.45)  &      &      &      &   &      &   \\
BiCut ($\alpha$=0.50)  &      &      &      &   &      &   \\
BiCut ($\alpha$=0.55)  &      &      &      &   &      &   \\
BiCut ($\alpha$=0.60)  &      &      &      &   &      &   \\
BiCut ($\alpha$=0.65)  &      &      &      &   &      &   \\
BiCut ($\alpha$=0.70)  &      &      &      &   &      &   \\
BiCut ($\alpha$=0.75)  &      &      &      &   &      &  \\
BiCut ($\alpha$=0.80) &      &      &      &   &      &   \\
\midrule
%Choppy ($\beta$=0) (50) & 892.72    & 0.746   &  &    &       &  \\
Choppy ($\beta$=0)  & 842.95     & 0.744   &  &  690.24  & 0.748      &  \\
%AttnCut ($\beta$=0) (50) &  922.16    &  0.746     &  &    &       &   \\
AttnCut ($\beta$=0) &  904.16    &  0.747     &  & 861.87  & 0.760      &   \\
%MtCut ($\beta$=0) (50) & 813.21   & 0.744      &  &    &       &  \\
MtCut ($\beta$=0)  & 843.67    & 0.741      &  & 745.44   & 0.747      &  \\
\midrule
%Choppy ($\beta$=0.5;$\alpha$=0.001) (50) & 451.88  & 0.743      &  &    &       &  \\
%Choppy ($\beta$=0.5;$\alpha$=0.001) (100)  & 479.56  & 0.743      &  &    &       &  \\
%AttnCut ($\beta$=0.5;$\alpha$=0.001) (50) &  773.77    &  0.743      &  &    &       &   \\
%AttnCut ($\beta$=0.5;$\alpha$=0.001) (100) &  713.21    &  0.744      &  &    &       &   \\
%MtCut ($\beta$=0.5;$\alpha$=0.001) (50) & 752.84    & 0.740      &  &    &       &  \\
%MtCut ($\beta$=0.5;$\alpha$=0.001) (100) & 687.00     & 0.741      &  &    &       &  \\
%\midrule
%Choppy ($\beta$=0.5;$\alpha$=0.005) (50) & 139.95     &  0.741     &  &    &       &  \\
%Choppy ($\beta$=0.5;$\alpha$=0.005) (100) & 161.12     &  0.738     &  &    &       &  \\
%AttnCut ($\beta$=0.5;$\alpha$=0.005) (50) & 44.21     & 0.673      &  &    &       &   \\
%AttnCut ($\beta$=0.5;$\alpha$=0.005) (100) & 62.84     & 0.693      &  &    &       &   \\
%MtCut ($\beta$=0.5;$\alpha$=0.005) &      &       &  &    &       &  \\
%MtCut ($\beta$=0.5;$\alpha$=0.005) &      &       &  &    &       &  \\
%\midrule
%Choppy ($\beta$=0.5;$\alpha$=0.01) (50) & 79.65  & 0.723     &  &    &       &  \\
%Choppy ($\beta$=0.5;$\alpha$=0.01) (100) & 71.44  & 0.718      &  &    &       &  \\
%AttnCut ($\beta$=0.5;$\alpha$=0.01) (50) & 27.88      & 0.643      &  &    &       &   \\
%AttnCut ($\beta$=0.5;$\alpha$=0.01) (100) & 40.40      & 0.674      &  &    &       &   \\
%MtCut ($\beta$=0.5;$\alpha$=0.01) &      &       &  &    &       &  \\
%\midrule
%Choppy ($\beta$=0.5;$\alpha$=0.05) (50) & 28.0     &  0.676     &  &    &       &  \\
%Choppy ($\beta$=0.5;$\alpha$=0.05) (100) & 26.51     &  0.667     &  &    &       &  \\
%AttnCut ($\beta$=0.5;$\alpha$=0.05) (50) & 32.70     & 0.565      &  &    &       &  \\
%AttnCut ($\beta$=0.5;$\alpha$=0.05) (100) & 11.26     & 0.562      &  &    &       &  \\
%MtCut ($\beta$=0.5;$\alpha$=0.05) &      &       &  &    &       &  \\
%\midrule
%Choppy ($\beta$=1;$\alpha$=0.001) (50) & 195.14    &  0.733    &  &    &       &  \\
$\alpha$=0.001 &  &  &  & & & \\
Choppy ($\beta$=1) & 140.63     &  0.733     &  & 89.65    & 0.696       &  \\
%AttnCut ($\beta$=1;$\alpha$=0.001) (50) &  272.74   & 0.718      &  &    &       &   \\
AttnCut ($\beta$=1) &  211.21    & 0.720      &  & 95.11    & 0.689      &   \\
%MtCut ($\beta$=1;$\alpha$=0.001) (50) & 356.37    &  0.726     &  &    &       &  \\
MtCut ($\beta$=1) & 138.26     &  0.714     &  & 130.98   & 0.696      &  \\
%Choppy ($\beta$=2;$\alpha$=0.001) (50) & 146.79    & 0.724     &  &    &       &  \\
Choppy ($\beta$=2)  & 118.84     & 0.732      &  & 52.67   &  0.661     &  \\
%AttnCut ($\beta$=2;$\alpha$=0.001) (50) &  49.51     &  0.688     &  &    &       &   \\
AttnCut ($\beta$=2)  &  64.16     &  0.692     &  & 63.89  & 0.681     &   \\
%MtCut ($\beta$=2;$\alpha$=0.001) (50) &  49.72   & 0.665     &  &    &       &  \\
MtCut ($\beta$=2) &  62.02    & 0.687      &  & 52.48   &  0.665     &  \\
\midrule
%Choppy ($\beta$=1;$\alpha$=0.005) (50) & 113.37    & 0.721     &  &    &       &  \\
%Choppy ($\beta$=1;$\alpha$=0.005) (100) & 62.28     & 0.686      &  &    &       &  \\
%AttnCut ($\beta$=1;$\alpha$=0.005) (50) & 34.60     & 0.660      &  &    &       &   \\
%AttnCut ($\beta$=1;$\alpha$=0.005) (100) &  43.02    &  0.677      &  &    &       &   \\
%MtCut ($\beta$=1;$\alpha$=0.005) (50) &  17.26    & 0.613      &  &    &       &  \\
%MtCut ($\beta$=1;$\alpha$=0.005) (100)& 38.53     & 0.650      &  &    &       &  \\
%\midrule
%Choppy ($\beta$=1;$\alpha$=0.01) (50) &  48.95   &  0.702    &  &    &       &  \\
$\alpha$=0.01 &  &  &  & & & \\
Choppy ($\beta$=1)  &  43.53   &  0.694    &  &  45.44  &  0.666     &  \\
%AttnCut ($\beta$=1;$\alpha$=0.01) (50)& 41.47     &  0.628     &  &    &       &   \\
AttnCut ($\beta$=1) & 26.58     &  0.653     &  & 35.06   &  0.639    &   \\
%MtCut ($\beta$=1;$\alpha$=0.01) (50) & 35.42     & 0.585      &  &    &       &  \\
MtCut ($\beta$=1)  & 41.30     & 0.613      &  & 30.09   & 0.615      &  \\
%Choppy ($\beta$=2;$\alpha$=0.01) (50) &  28.19    & 0.674      &  &    &       &  \\
Choppy ($\beta$=2)  &  27.67    & 0.670      &  & 29.17   &  0.627     &  \\
%AttnCut ($\beta$=2;$\alpha$=0.01) (50) & 36.37     & 0.599     &  &    &       &   \\
AttnCut ($\beta$=2)  & 38.35     & 0.617      &  & 24.24   & 0.625      &   \\
%MtCut ($\beta$=2;$\alpha$=0.01) (50)  & 34.09     &  0.579     &  &    &       &  \\
MtCut ($\beta$=2)  & 36.58     & 0.593      &  & 18.09   & 0.595     &  \\
\midrule
$\alpha$=0.05 &  &  &  & & & \\
%Choppy ($\beta$=1;$\alpha$=0.05) (50) & 14.0   & 0.605    &  &    &       &  \\
Choppy ($\beta$=1)  & 14.0   & 0.605    &  & 21.26   &  0.613     &  \\
%AttnCut ($\beta$=1;$\alpha$=0.05) (50)& 8.65    & 0.549     &  &    &       &   \\
AttnCut ($\beta$=1) & 9.44     & 0.545      &  &  9.87  & 0.531      &   \\
%MtCut ($\beta$=1;$\alpha$=0.05) (50) &  121.4    &  0.594     &  &    &       &  \\
MtCut ($\beta$=1)  & 32.70     &  0.565     &  &  11.61  &  0.559     &  \\
%Choppy ($\beta$=2;$\alpha$=0.05) (50) & 14.0     &  0.605   &  &    &       &  \\
Choppy ($\beta$=2)  & 14.0     &  0.605   &  & 16.52   & 0.603       &  \\
%AttnCut ($\beta$=2;$\alpha$=0.05) (50) & 7.07    & 0.542    &  &    &       &   \\
AttnCut ($\beta$=2)  & 8.51   & 0.544      &  & 8.65  & 0.519      &   \\
%MtCut ($\beta$=2;$\alpha$=0.05) (50) & 7.88     & 0.550      &  &    &       &  \\
MtCut ($\beta$=2)  & 8.51     &  0.555      &  &  7.57  & 0.536      &  \\
%Choppy ($\beta$=2;$\alpha$=0.005) (50) &  44.65   &  0.698    &  &    &       &  \\
%Choppy ($\beta$=2;$\alpha$=0.005) (100) &  44.93    &  0.689     &  &    &       &  \\
%AttnCut ($\beta$=2;$\alpha$=0.005) (50)& 24.33     & 0.640      &  &    &       &   \\
%AttnCut ($\beta$=2;$\alpha$=0.005) (100)& 30.84      & 0.653      &  &    &       &   \\
%MtCut ($\beta$=2;$\alpha$=0.005)  &      &       &  &    &       &  \\
\midrule
  Oracle-$k$ & 156.88  &  0.785  &   & 228.56  & 0.804  &  \\
\bottomrule
\end{tabular}
%}
\end{table}


\begin{table}[!t]
\centering
\caption{
A comparison of \ac{RLT} methods, optimized to maximize F1 and DCG of the retrieved list returned by BM25, in predicting re-ranking cut-off points for the BM25--RankLLaMA pipeline on TREC-DL 19 and 20.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l lll lll} 
\toprule
 \multirow{2}{*}{Method} & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \multicolumn{1}{c}{\small{Avg. k}} & \multicolumn{1}{c}{\small{nDCG@10}}     & \multicolumn{1}{c}{\small{Lat.}}  & \multicolumn{1}{c}{\small{Avg. k}}   & \multicolumn{1}{c}{\small{nDCG@10}}    & \multicolumn{1}{c}{\small{Lat.}}     \\
\midrule
w/o re-ranking & -  & 0.506     & -   & -   & 0.480  & -   \\
  \midrule
  Fixed-$k$ (10) & 10   & 0.557    &  & 10  &  0.532  &      \\
  Fixed-$k$ (100) & 20   & 0.651    &  &  20 & 0.612   &  \\
  Fixed-$k$ (100) & 100  & 0.730    &  & 100  & 0.697  &    \\
   Fixed-$k$ (200) & 200  & 0.739   &  & 200  & 0.719  &   \\
 %$k=300$ & 300  & 0.739   &  & 300 & 0.731  &    \\
 %$k=400$ & 400  & 0.741    &  & 400  & 0.733  &  \
 %$k=500$ & 500   & 0.745   &  & 500 & 0.739  &   \\
% $k=600$ & 600  &  0.743    &  & 600 & 0.750  &   \\
Fixed-$k$ (1000)  & 1000  & 0.747    &  & 1000  &  0.762 &  \\
Greedy-$k$ (DCG) &      &       &  &    &       &      \\
Surprise (DCG) &      &       &  &    &       &   \\
Greedy-$k$ (F1) &      &       &  &    &       &      \\
Surprise (F1) &      &       &  &    &       &   \\

\midrule
BiCut ($\alpha$=0.40)  & 385.51  & 0.739   &  & 537.57   & 0.745  & \\
BiCut ($\alpha$=0.45)  & 168.40  & 0.729   &  &  501.56  & 0.741  & \\
BiCut ($\alpha$=0.50)  & 184.02  & 0.729   &  & 361.59   & 0.716  & \\
BiCut ($\alpha$=0.55)  & 130.49  & 0.688   &  & 412.59   & 0.723  & \\
BiCut ($\alpha$=0.60)  & 130.74  & 0.693   &  & 340.81   & 0.705  & \\
BiCut ($\alpha$=0.65)  & 99.09  & 0.684   &  & 204.69   & 0.692  & \\
Choppy (DCG)  & 2.16  & 0.514 &  &  6.04 &  0.497  & \\
AttnCut (DCG) & 1.23  & 0.507 &  & 1.74  &  0.488  & \\
MtCut (DCG) & 1.00  & 0.506 &  & 1.22  & 0.480  & \\
Choppy (F1)   &  34.56    & 0.648     &  &  33.61 &  0.607    &  \\
AttnCut (F1) &  12.56     &  0.577     &   & 30.31   &0.625     &     \\
MtCut (F1) &  10.23    & 0.568      &  & 36.33    & 0.630    &    \\
\midrule
% Oracle fixed-k & 991  & 0.747    &   &  987 &  0.762  &  \\
 Oracle-$k$ & 156.88  &  0.785  &   & 228.56  & 0.804  &  \\
\bottomrule
\end{tabular}
%}
\end{table}

\begin{table}[!t]
\centering
\caption{
A comparison of \ac{RLT} methods, optimized to maximize F1 and DCG of the retrieved list returned by BM25, in predicting re-ranking cut-off points for the SPLADE++--RankLLaMA pipeline on TREC-DL 19 and 20.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l lll lll} 
\toprule
 \multirow{2}{*}{Method} & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20} \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \multicolumn{1}{c}{Avg. k} & \multicolumn{1}{c}{nDCG@10}     & \multicolumn{1}{c}{Lat.}   & \multicolumn{1}{c}{Avg. k}   & \multicolumn{1}{c}{nDCG@10}   & \multicolumn{1}{c}{Lat.}      \\
\midrule
$k=0$ &  0  &  0.731  &   & 0   & 0.720    &   \\
  \midrule
 $k=10 $ & 10  & 0.740   &   & 10  & 0.741   &   \\
 $k=20 $ & 20  & 0.773   &   & 20  & 0.778   &    \\
 $k=100$ & 100  & 0.769   &   & 100  & 0.771   &  \\
 $k=200$ & 200   & 0.769   &   & 200  & 0.769   &  \\
 $k=1000$ & 1000    & 0.768   &   & 1000  & 0.768   &   \\
 Greedy  &    &    &   &   &    & \\
 Surprise &    &    &   &   &    &  \\
\midrule
BiCut &    &    &   &   &    &  \\
Choppy   &    &    &   &   &    &  \\
AttnCut &    &    &   &   &    &  \\
MtCut &    &    &   &   &    &  \\
\midrule
 Oracle-$k$& 17.44   & 0.810   &    & 27.69  & 0.82    & \\
\bottomrule
\end{tabular}
%}
\end{table}

\begin{table}[!t]
\centering
\caption{
A comparison of \ac{RLT} methods, optimized to maximize F1 and DCG of the retrieved list returned by BM25, in predicting re-ranking cut-off points for the RepLLaMA--RankLLaMA pipeline on TREC-DL 19 and 20.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l lll lll} 
\toprule
 \multirow{2}{*}{Method} & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20} \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \multicolumn{1}{c}{Avg. k} & \multicolumn{1}{c}{nDCG@10}     & \multicolumn{1}{c}{Latency}   & \multicolumn{1}{c}{Avg. k}   & \multicolumn{1}{c}{nDCG@10}   & \multicolumn{1}{c}{Lat.}      \\
\midrule
$k=0$ & 0 & 0.738      &   & 0 & 0.720    &    \\
  \midrule
 $k=10 $ & 10  & 0.742   &    & 10   &  0.729    &    \\
 $k=20 $ & 20  & 0.765   &     & 20    & 0.761     &    \\
 $k=100$ & 100  & 0.769    &    & 100  &  0.767   &   \\
 $k=200$ & 200  & 0.768    &     & 200   & 0.768  &   \\
 $k=1000$ & 1000  & 0.763    &     & 1000   & 0.768  &   \\
 Greedy  &        &    &       &     &     &  \\
 Surprise &      &       &  &    &       &   \\
\midrule
BiCut & 166.81   & 0.766   &       &  322.50   &  0.768    &  \\
Choppy   & 12.33   & 0.744   &       &  70.35   &  0.765   &  \\
AttnCut &  18.23    & 0.752    &   & 31.52    & 0.760     &  \\
MtCut & 3.42     &  0.733   &       &  16.13   & 0.730    &  \\
LeCut &              &    &       &     &     &  \\
\midrule
% Oracle fixed-k &  126  & 0.770 &   &   & 50   &  0.769 &   & \\
 Oracle-$k$ & 23.33   & 0.794     &   & 42.46  &  0.799   & \\
\bottomrule
\end{tabular}
%}
\end{table}





\begin{table}[!t]
\centering
\caption{
sanity check
A comparison of \ac{RLT} methods, optimized to maximize F1 and DCG of the retrieved list returned by BM25, in predicting re-ranking cut-off points for the BM25--RankLLaMA pipeline on TREC-DL 19 and 20.
}
\label{tab:finetuning}
\setlength{\tabcolsep}{1mm}
\begin{tabular}{l lll lll} 
\toprule
 \multirow{2}{*}{Method} & \multicolumn{3}{c}{TREC-DL 19} & \multicolumn{3}{c}{TREC-DL 20}  \\
  \cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \multicolumn{1}{c}{\small{Avg. k}} & \multicolumn{1}{c}{\small{nDCG@10}}     & \multicolumn{1}{c}{\small{Lat.}}  & \multicolumn{1}{c}{\small{Avg. k}}   & \multicolumn{1}{c}{\small{nDCG@10}}    & \multicolumn{1}{c}{\small{Lat.}}     \\
  \midrule
  Fixed-$k$ (10) &   &    &  &    &   & \\    
  Fixed-$k$ (100) &   &    &  &    &   & \\ 
  Fixed-$k$ (100) &   &    &  &    &   & \\  
   Fixed-$k$ (200) &   &    &  &    &   & \\ 
Fixed-$k$ (1000)  &   &    &  &    &   & \\ 
Greedy-$k$ (DCG) &      &       &  &    &       &      \\
Surprise (DCG) &      &       &  &    &       &   \\
Greedy-$k$ (F1) &      &       &  &    &       &      \\
Surprise (F1) &      &       &  &    &       &   \\
\midrule
BiCut ($\alpha$=0.40)  &   &    &  &    &   & \\
BiCut ($\alpha$=0.45)  &   &    &  &    &   & \\
BiCut ($\alpha$=0.50)  &   &    &  &    &   & \\ 
BiCut ($\alpha$=0.55) &   &    &  &    &   & \\
BiCut ($\alpha$=0.60)  &   &    &  &    &   & \\
BiCut ($\alpha$=0.65)  &   &    &  &    &   & \\
Choppy (DCG)  &   &    &  &    &   & \\ 
AttnCut (DCG)  &   &    &  &    &   & \\
MtCut (DCG) &   &    &  &    &   & \\ 
Choppy (F1)   &   &    &  &    &   & \\  
AttnCut (F1) &   &    &  &    &   & \\     
MtCut (F1) &   &    &  &    &   & \\    
\midrule
 Oracle-$k$ &   &    &  &    &   & \\  
\bottomrule
\end{tabular}
%}
\end{table}



the ability of our framework to select a more optimal operating point in the space of effectiveness-efficiency tradeoffs

\begin{table}[h]
\centering
\caption{Data statistics of TREC-DL 19 and 20, retrieval quality of BM25, SPLADE++ and RepLLaMA and re-ranking quality of RankLLaMA with   the retrievers in terms of nDCG@10. The number in brackets indicate the re-ranking cut-off..}
\label{table:dl19-20}
\begin{tabular}{l cc}
\toprule
& TREC-DL 19  & TREC-DL 20 \\ 
\midrule
BM25  & 0.506   & 0.480  \\ 
SPLADE++   & 0.731    & 0.720 \\
RepLLaMA  & 0.738    & 0.720  \\ 
\midrule 
BM25--RankLLaMA (200)   & 0.739    & 0.804 \\
SPLADE++--RankLLaMA (200)   & 0.769    & 0.769 \\
RepLLaMA--RankLLaMA (200)   & 0.769    & 0.768 \\
\midrule 
BM25--RankLLaMA (oracle)   & 0.785    & 0.719 \\
SPLADE++--RankLLaMA (oracle)   & 0.810   & 0.820 \\
RepLLaMA--RankLLaMA (oracle)   & 0.794    & 0.799  \\
\midrule 
\# queries & 43  & 54   \\
%\#passages & \multicolumn{2}{c}{8.8M}  \\ 
\bottomrule
\end{tabular}
%}
\end{table}

\header{Baselines}
We consider three groups of baselines:
\begin{enumerate*}[label=(\roman*)]
    \item Fixed-k 
    \item Greedy
    \item \ac{QPP}-based \acf{VDP}
    \item ranked list truncation,
    \item candidate pruning,
    %\item re-ranking early stopping,
    \item oracle methods,
\end{enumerate*} 


quantify the tradeoff between retrieval effectiveness 

estimate the minimize re-ranking depth, on a per-query basis, that leads to the highest re-ranking performance.

Among all the truncation methods, Fix-k always performs the worst.

it means returning a fixed number of results cannot guarantee a good trade-off between user efforts and the overall utility over retrieval results.~\citep{wang2022mtcut}
Although Greedy seems to have good results, the performance of such a cut-off method depends on the consistency between the training set and test set entirely~\citep{ma2022incorporating} 
%
Candidate set pruning has been commonly used to speed up two-stage relevance ranking~\citep{li2022certified}.

\citet{culpepper2016dynamic} state that increasingly expensive re-ranking steps may require processing fewer and fewer documents 



little attention has been paid to the effect that these approaches have on query execution time
 
Existing work studying into \ac{LLM}-based re-ranking usually follows a standard ``retrieve-then-rerank'' setup and sets a fixed re-ranking depth applied to all queries.
E.g., \citet{ma2023fine} employ the \ac{LLM}-based re-ranker RankLLaMA to reorder the top 200 items returned by the \ac{LLM}-based retriever RepLLaMA.   
However, our empirical analysis based on two retrievers and two \ac{LLM}-based re-rankers shows that applying a fixed re-ranking depth to all queries leads to sub-optimal re-ranking performance and many unnecessary computational costs.

retrieving the same number of candidates for all queries in a cascade architecture is not appropriate, and, in fact, individual queries may require a shorter or a longer list of candidates


\Acp{LLM} have demonstrated impressive performance on various \ac{IR} and \ac{NLP} tasks~\citep{zhu2023large,zhao2023survey}. 
Applying \acp{LLM} to re-ranking has attracted growing interest, 
%

Work in \ac{LLM}-based re-ranking has focused on improving re-ranking effectiveness while improving the efficiency of \ac{LLM}-based re-ranking has received less attention.


Ranked list truncation serves as a prerequisite for retrieval systems with multiple stages because in such systems, the highly-effective model at the second stage is usually computationally expensive~\citep{ma2022incorporating,lien2019assumption}
 \citet{zamani2022stochastic}

re-ranking efficiency has received much attention since pre-trained language models (e.g., BERT~\citep{devlin2019bert}) are employed as re-rankers~\citep{nogueira2019passage}; BERT-based re-rankers have been reported to be slower than classical re-rankers by orders of magnitude~\citep{hofstatter2019let}, making them hard to be applied in practical applications; 

RepLLaMA–RankLLaMA pipeline 

determining the optimal rank cut-off values
 
 pairwise approaches may elevate a poorly ranked relevant document to a high position

 promoting several poorly ranked relevant documents into higher positions.

neural truncation methods (i.e., BiCut and Choppy) can achieve better results than the traditional truncation methods

perform better for neural-based a retriever than lexical retriever


This is expected since larger k translates into higher recall at the candidate generation stage, i.e., more relevant documents are available to the reranker.

documents with a relatively low BM25 score can indeed be relevant to the query and be placed at higher ranks with monoBERT


reducing expensive neural re-ranking is where most of our speedups come from

these gains have come at substantial costs in terms of efficiency,

attains impressive efficiency benefits while still attaining high effectiveness

optimizing effectiveness-efficiency tradeoffs on a per-query basis,

 marked improvements in efficiency can be obtained while ensuring effectiveness

without negatively impacting effectiveness.

up to 40\% reduction in response time

this results in a 2.65× speedup

a fixed cutoff baseline

as plotted in Figure 2

the truth documents are not uniformly distributed. 

the higher the re-ranking depth the higher the full system latency

reduce the re-ranking cost without a significant change in re-ranking effectiveness.

achieve a better tradeoff between accuracy and efficiency.

maintaining acceptable effectiveness/efficiency tradeoffs

computationally demanding

speeding-up the exploitation of tree ensembles without hindering their effectiveness. 

up to a 42×speedup on web document ranking



xx can accelerate model inference by up to x\% with minimal model quality degradation. 

directly optimize the tradeoff between effectiveness and efficiency

strike a balance between effectiveness and efficiency


The exact value of t can be set depending on which direction a user wishes to bias the tradeoff.  

Choosing a higher t biases the tradeoff in the effectiveness direction

Candidate Set Pruning
early exit
early stopping
dynamic cutoff prediction 
candidate generation stage

The objective of \ac{QPP} is not exactly the same as the objective of a downstream task.

questions raised by interviewers.  

These models can be leveraged to directly generate a reordered list of candidates

in descending order of relevance
in decreasing order of relevance

the LLM is prompted to 


computationally expensive
computationally intensive
a considerable computational overhead


we propose to make xx a function of xx

Herein = in this paper


produces a ranking over the corpus


a pair of a query and a retrieval method entails a retrieved list
